Modelling Domain Relationships for Transfer Learning on Retrieval-based Question Answering Systems in E-commerce

In this paper, we study transfer learning for the PI and NLI problems, aiming to propose a general framework, which can effectively and efficiently adapt the shared knowledge learned from a resource-rich source domain to a resource- poor target domain. Specifically, since most existing transfer learning methods only focus on learning a shared feature space across domains while ignoring the relationship between the source and target domains, we propose to simultaneously learn shared representations and domain relationships in a unified framework. Furthermore, we propose an efficient and effective hybrid model by combining a sentence encoding- based method and a sentence interaction-based method as our base model. Extensive experiments on both paraphrase identification and natural language inference demonstrate that our base model is efficient and has promising performance compared to the competing models, and our transfer learning method can help to significantly boost the performance. Further analysis shows that the inter-domain and intra-domain relationship captured by our model are insightful. Last but not least, we deploy our transfer learning model for PI into our online chatbot system, which can bring in significant improvements over our existing system. Finally, we launch our new system on the chatbot platform Eva in our E-commerce site AliExpress.

==> sample <==
@InProceedings{alime-demo,
  Title                    = {AliMe Assist: An Intelligent Assistant for Creating an Innovative E-commerce Experience},
  Author                   = {Li, Feng-Lin and Qiu, Minghui and Chen, Haiqing and Wang, Xiongwei and Gao, Xing and Huang, Jun and Ren, Juwei and Zhao, Zhongzhou and Zhao, Weipeng and Wang, Lei and Jin, Guwei},
  Booktitle                = {CIKM 2017. Demo},
  Year                     = {2017}
}

@InProceedings{argyriou:nips2007,
  Title                    = {Multi-task feature learning},
  Author                   = {Argyriou, Andreas and Evgeniou, Theodoros and Pontil, Massimiliano},
  Booktitle                = {NIPS},
  Year                     = {2007}
}

@InProceedings{blitzer:EMNLP2006,
  Title                    = {Domain Adaptation with Structural Correspondence Learning},
  Author                   = {Blitzer, John and McDonald, Ryan and Pereira, Fernando},
  Booktitle                = {EMNLP},
  Year                     = {2006}
}

@InProceedings{bowman:acl2016,
  Title                    = {A Fast Unified Model for Parsing and Sentence Understanding},
  Author                   = {Bowman, Samuel R. and Gauthier, Jon and Rastogi, Abhinav and Gupta, Raghav and Manning, Christopher D. and Potts, Christopher},
  Booktitle                = {ACL},
  Year                     = {2016}
}

@Article{bradley:pr1997,
  Title                    = {The use of the area under the ROC curve in the evaluation of machine learning algorithms},
  Author                   = {Bradley, Andrew P},
  Journal                  = {Pattern recognition},
  Year                     = {1997},
  Number                   = {7},
  Pages                    = {1145--1159},
  Volume                   = {30},
  Publisher                = {Elsevier}
}

@InProceedings{callison:emnlp2008,
  Title                    = {Syntactic constraints on paraphrases extracted from parallel corpora},
  Author                   = {Callison-Burch, Chris},
  Booktitle                = {EMNLP},
  Year                     = {2008}
}

@InProceedings{chen:acl2017,
  Title                    = {Enhanced LSTM for Natural Language Inference},
  Author                   = {Chen, Qian and Zhu, Xiaodan and Ling, Zhen-Hua and Wei, Si and Jiang, Hui and Inkpen, Diana},
  Booktitle                = {ACL},
  Year                     = {2017}
}

@InProceedings{cui:acl17,
  Title                    = {SuperAgent: A Customer Service Chatbot for E-commerce Websites},
  Author                   = {Cui, Lei and Huang, Shaohan and Wei, Furu and Tan, Chuanqi and Duan, Chaoqun and Zhou, Ming},
  Booktitle                = {ACL 2017, Demo},
  Year                     = {2017}
}

@InProceedings{dai:icml2007,
  Title                    = {Boosting for transfer learning},
  Author                   = {Dai, Wenyuan and Yang, Qiang and Xue, Gui-Rong and Yu, Yong},
  Booktitle                = {ICML},
  Year                     = {2007}
}

@InProceedings{daumeiii:acl2007,
  Title                    = {Frustratingly Easy Domain Adaptation},
  Author                   = {Daume III, Hal},
  Booktitle                = {ACL},
  Year                     = {2007}
}

@Article{duchi:jmlr2011,
  Title                    = {Adaptive subgradient methods for online learning and stochastic optimization},
  Author                   = {Duchi, John and Hazan, Elad and Singer, Yoram},
  Journal                  = {Journal of Machine Learning Research},
  Year                     = {2011},
  Number                   = {Jul},
  Pages                    = {2121--2159},
  Volume                   = {12}
}

@InProceedings{fader:ACL2013,
  Title                    = {Paraphrase-Driven Learning for Open Question Answering},
  Author                   = {Fader, Anthony and Zettlemoyer, Luke and Etzioni, Oren},
  Booktitle                = {ACL},
  Year                     = {2013}
}

@Article{ganin:jmlr2016,
  Title                    = {Domain-adversarial training of neural networks},
  Author                   = {Ganin, Yaroslav and Ustinova, Evgeniya and Ajakan, Hana and Germain, Pascal and Larochelle, Hugo and Laviolette, Fran{\c{c}}ois and Marchand, Mario and Lempitsky, Victor},
  Journal                  = {Journal of Machine Learning Research},
  Year                     = {2016},
  Number                   = {59},
  Pages                    = {1--35},
  Volume                   = {17}
}

@InProceedings{gillick:icassp1989,
  Title                    = {Some statistical issues in the comparison of speech recognition algorithms},
  Author                   = {Gillick, Laurence and Cox, Stephen J},
  Booktitle                = {ICASSP},
  Year                     = {1989}
}

@InProceedings{goodfellow:nips2014,
  Title                    = {Generative adversarial nets},
  Author                   = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  Booktitle                = {NIPS},
  Year                     = {2014}
}

@InProceedings{hu:nips2014,
  Title                    = {Convolutional neural network architectures for matching natural language sentences},
  Author                   = {Hu, Baotian and Lu, Zhengdong and Li, Hang and Chen, Qingcai},
  Booktitle                = {NIPS},
  Year                     = {2014}
}

@InProceedings{jeon:cikm2005,
  Title                    = {Finding similar questions in large question and answer archives},
  Author                   = {Jeon, Jiwoon and Croft, W Bruce and Lee, Joon Ho},
  Booktitle                = {CIKM},
  Year                     = {2005}
}

@InProceedings{jiang:acl2007,
  Title                    = {Instance Weighting for Domain Adaptation in NLP},
  Author                   = {Jiang, Jing and Zhai, ChengXiang},
  Booktitle                = {ACL},
  Year                     = {2007}
}

@InProceedings{kim:emnlp2014,
  Title                    = {Convolutional Neural Networks for Sentence Classification},
  Author                   = {Kim, Yoon},
  Booktitle                = {EMNLP},
  Year                     = {2014}
}

@InProceedings{kusner:icml2015,
  Title                    = {From word embeddings to document distances},
  Author                   = {Kusner, Matt and Sun, Yu and Kolkin, Nicholas and Weinberger, Kilian},
  Booktitle                = {ICML},
  Year                     = {2015}
}

@InProceedings{lee:icml2007,
  Title                    = {Learning a meta-level prior for feature relevance from multiple related tasks},
  Author                   = {Lee, Su-In and Chatalbashev, Vassil and Vickrey, David and Koller, Daphne},
  Booktitle                = {ICML},
  Year                     = {2007}
}

@InProceedings{liu:acl2017,
  Title                    = {Adversarial Multi-task Learning for Text Classification},
  Author                   = {Liu, Pengfei and Qiu, Xipeng and Huang, Xuanjing},
  Booktitle                = {ACL},
  Year                     = {2017}
}

@InProceedings{liu:kdd2017,
  Title                    = {Distributed Multi-Task Relationship Learning},
  Author                   = {Liu, Sulin and Pan, Sinno Jialin and Ho, Qirong},
  Booktitle                = {KDD},
  Year                     = {2017}
}

@Article{long:tkde2014,
  Title                    = {Adaptation regularization: A general framework for transfer learning},
  Author                   = {Long, Mingsheng and Wang, Jianmin and Ding, Guiguang and Pan, Sinno Jialin and Philip, S Yu},
  Journal                  = {IEEE Transactions on Knowledge and Data Engineering},
  Year                     = {2014},
  Number                   = {5},
  Pages                    = {1076--1089},
  Volume                   = {26},
  Publisher                = {IEEE}
}

@InProceedings{mou:acl2016,
  Title                    = {Natural Language Inference by Tree-Based Convolution and Heuristic Matching},
  Author                   = {Mou, Lili and Men, Rui and Li, Ge and Xu, Yan and Zhang, Lu and Yan, Rui and Jin, Zhi},
  Booktitle                = {ACL},
  Year                     = {2016}
}

@InProceedings{mou:EMNLP2016,
  Title                    = {How Transferable are Neural Networks in NLP Applications?},
  Author                   = {Mou, Lili and Meng, Zhao and Yan, Rui and Li, Ge and Xu, Yan and Zhang, Lu and Jin, Zhi},
  Booktitle                = {EMNLP},
  Year                     = {2016}
}

@InProceedings{napoles:aclw2011,
  Title                    = {Paraphrastic sentence compression with a character-based metric: Tightening without deletion},
  Author                   = {Napoles, Courtney and Callison-Burch, Chris and Ganitkevitch, Juri and Van Durme, Benjamin},
  Booktitle                = {Proceedings of the Workshop on Monolingual Text-To-Text Generation},
  Year                     = {2011}
}

@Article{pan:tkde2010,
  Title                    = {A survey on transfer learning},
  Author                   = {Pan, Sinno Jialin and Yang, Qiang},
  Journal                  = {IEEE Transactions on knowledge and data engineering},
  Year                     = {2010},
  Number                   = {10},
  Pages                    = {1345--1359},
  Volume                   = {22},
  Publisher                = {IEEE}
}

@InProceedings{pang:aaai2016,
  Title                    = {Text Matching as Image Recognition},
  Author                   = {Pang, Liang and Lan, Yanyan and Guo, Jiafeng and Xu, Jun and Wan, Shengxian and Cheng, Xueqi},
  Booktitle                = {AAAI},
  Year                     = {2016}
}

@InProceedings{parikh:emnlp2016,
  Title                    = {A Decomposable Attention Model for Natural Language Inference},
  Author                   = {Parikh, Ankur and T\"{a}ckstr\"{o}m, Oscar and Das, Dipanjan and Uszkoreit, Jakob},
  Booktitle                = {EMNLP},
  Year                     = {2016}
}

@InProceedings{pennington:emnlp2014,
  Title                    = {GloVe: Global Vectors for Word Representation},
  Author                   = {Jeffrey Pennington and Richard Socher and Christopher D. Manning},
  Booktitle                = {EMNLP},
  Year                     = {2014}
}

@InProceedings{qiu:acl17,
  Title                    = {AliMe Chat: A Sequence to Sequence and Rerank based Chatbot Engine},
  Author                   = {Qiu, Minghui and Li, Feng-Lin and Wang, Siyu and Gao, Xing and Chen, Yan and Zhao, Weipeng and Chen, Haiqing and Huang, Jun and Chu, Wei},
  Booktitle                = {ACL},
  Year                     = {2017}
}

@InProceedings{qiu:icdm2017,
  Title                    = {A Short-Term Rainfall Prediction Model using Multi-Task Convolutional Neural Networks.},
  Author                   = {Qiu, Minghui and Zhao, Peilin and Zhang, Ke and Huang, Jun and Shi, Xing and Wang, Xiaoguang and Chu, Wei},
  Booktitle                = {ICDM},
  Year                     = {2017}
}

@Article{robertson:ir2009,
  Title                    = {The probabilistic relevance framework: BM25 and beyond},
  Author                   = {Robertson, Stephen and Zaragoza, Hugo and others},
  Journal                  = {Foundations and Trends{\textregistered} in Information Retrieval},
  Year                     = {2009},
  Number                   = {4},
  Pages                    = {333--389},
  Volume                   = {3}
}

@Article{rock:iclr2015,
  Title                    = {Reasoning about entailment with neural attention},
  Author                   = {Rockt{\"a}schel, Tim and Grefenstette, Edward and Hermann, Karl Moritz and Ko{\v{c}}isk{\`y}, Tom{\'a}{\v{s}} and Blunsom, Phil},
  Journal                  = {ICLR},
  Year                     = {2015}
}

@InProceedings{snli:emnlp2015,
  Title                    = {A large annotated corpus for learning natural language inference},
  Author                   = {Bowman, Samuel R. and Angeli, Gabor and Potts, Christopher, and Manning, Christopher D.},
  Booktitle                = {EMNLP},
  Year                     = {2015}
}

@InProceedings{socher:nips2011,
  Title                    = {Dynamic pooling and unfolding recursive autoencoders for paraphrase detection},
  Author                   = {Socher, Richard and Huang, Eric H and Pennin, Jeffrey and Manning, Christopher D and Ng, Andrew Y},
  Booktitle                = {NIPS},
  Year                     = {2011}
}

@Article{taigman:iclr2017,
  Title                    = {Unsupervised cross-domain image generation},
  Author                   = {Taigman, Yaniv and Polyak, Adam and Wolf, Lior},
  Journal                  = {ICLR},
  Year                     = {2017}
}

@Article{takagi:semeval2015,
  Title                    = {WSL: Sentence Similarity Using Semantic Distance Between Words},
  Author                   = {Takagi, Naoko Miura Tomohiro},
  Journal                  = {SemEval-2015},
  Year                     = {2015}
}

@Article{vinyals:arxiv2015,
  Title                    = {A neural conversational model},
  Author                   = {Vinyals, Oriol and Le, Quoc},
  Journal                  = {arXiv preprint arXiv:1506.05869},
  Year                     = {2015}
}

@InProceedings{wang:acl2015,
  Title                    = {A Long Short-Term Memory Model for Answer Sentence Selection in Question Answering},
  Author                   = {Wang, Di and Nyberg, Eric},
  Booktitle                = {ACL-IJCNLP},
  Year                     = {2015}
}

@InProceedings{wang:apsipa2015,
  Title                    = {Transfer learning for speech and language processing},
  Author                   = {Wang, Dong and Zheng, Thomas Fang},
  Booktitle                = {Signal and Information Processing Association Annual Summit and Conference (APSIPA)},
  Year                     = {2015}
}

@Article{wang:iclr2017,
  Title                    = {A Compare-Aggregate Model for Matching Text Sequences},
  Author                   = {Wang, Shuohang and Jiang, Jing},
  Journal                  = {ICLR},
  Year                     = {2017}
}

@InProceedings{wang:icml2008,
  Title                    = {Manifold alignment using procrustes analysis},
  Author                   = {Wang, Chang and Mahadevan, Sridhar},
  Booktitle                = {ICML},
  Year                     = {2008}
}

@InProceedings{wang:naacl2016,
  Title                    = {Learning Natural Language Inference with LSTM},
  Author                   = {Wang, Shuohang and Jiang, Jing},
  Booktitle                = {NAACL-HLT},
  Year                     = {2016}
}

@InProceedings{wang:wsdm2017,
  Title                    = {Concept Embedded Convolutional Semantic Model for Question Retrieval},
  Author                   = {Wang, Pengwei and Zhang, Yong and Ji, Lei and Yan, Jun and Jin, Lianwen},
  Booktitle                = {WSDM},
  Year                     = {2017}
}

@Article{wieting:iclr2016,
  Title                    = {Towards universal paraphrastic sentence embeddings},
  Author                   = {Wieting, John and Bansal, Mohit and Gimpel, Kevin and Livescu, Karen},
  Journal                  = {ICLR},
  Year                     = {2016}
}

@Article{williams:arxiv2017,
  Title                    = {A Broad-Coverage Challenge Corpus for Sentence Understanding through Inference},
  Author                   = {Williams, Adina and Nangia, Nikita and Bowman, Samuel R},
  Journal                  = {arXiv preprint arXiv:1704.05426},
  Year                     = {2017}
}

@Article{wu:tois2008,
  Title                    = {Interpreting tf-idf term weights as making relevance decisions},
  Author                   = {Wu, Ho Chung and Luk, Robert Wing Pong and Wong, Kam Fai and Kwok, Kui Lam},
  Journal                  = {ACM Transactions on Information Systems (TOIS)},
  Year                     = {2008},
  Number                   = {3},
  Pages                    = {13},
  Volume                   = {26},
  Publisher                = {ACM}
}

@InProceedings{yan:sigir2016,
  Title                    = {Learning to respond with deep neural networks for retrieval-based human-computer conversation system},
  Author                   = {Yan, Rui and Song, Yiping and Wu, Hua},
  Booktitle                = {SIGIR},
  Year                     = {2016}
}

@Article{yang:iclr2017,
  Title                    = {Transfer learning for sequence tagging with hierarchical recurrent networks},
  Author                   = {Yang, Zhilin and Salakhutdinov, Ruslan and Cohen, William W},
  Journal                  = {ICLR},
  Year                     = {2017}
}

@InProceedings{yin:naacl2015,
  Title                    = {Convolutional Neural Network for Paraphrase Identification.},
  Author                   = {Yin, Wenpeng and Sch{\"u}tze, Hinrich},
  Booktitle                = {NAACL-HLT},
  Year                     = {2015}
}

@Article{yin:tacl2016,
  Title                    = {ABCNN: Attention-Based Convolutional Neural Network for Modeling Sentence Pairs},
  Author                   = {Yin, Wenpeng and Sch{\"u}tze, Hinrich and Xiang, Bing and Zhou, Bowen},
  Journal                  = {Transactions of ACL},
  Year                     = {2016},
  Pages                    = {259--272},
  Volume                   = {4}
}

@InProceedings{yosinski:nips2014,
  Title                    = {How transferable are features in deep neural networks?},
  Author                   = {Yosinski, Jason and Clune, Jeff and Bengio, Yoshua and Lipson, Hod},
  Booktitle                = {NIPS},
  Year                     = {2014}
}

@InProceedings{yu:EMNLP2016,
  Title                    = {Learning Sentence Embeddings with Auxiliary Tasks for Cross-Domain Sentiment Classification},
  Author                   = {Yu, Jianfei and Jiang, Jing},
  Booktitle                = {EMNLP},
  Year                     = {2016}
}

@InProceedings{zhang:uai2010,
  Title                    = {A convex formulation for learning task relationships in multi-task learning},
  Author                   = {Zhang, Yu and Yeung, Dit-Yan},
  Booktitle                = {UAI},
  Year                     = {2010}
}

@Article{zhou:tkde2017,
  Title                    = {Modeling and Learning Distributed Word Representation with Metadata for Question Retrieval},
  Author                   = {Zhou, Guangyou and Huang, Jimmy Xiangji},
  Journal                  = {IEEE Transactions on Knowledge and Data Engineering},
  Year                     = {2017},
  Number                   = {6},
  Pages                    = {1226--1239},
  Volume                   = {29},
  Publisher                = {IEEE}
}

@comment{jabref-meta: databaseType:biblatex;}


